Distributed estimation from relative measurements of heterogeneous and uncertain quality

This paper studies the problem of estimation from relative measurements in a graph, in which a vector indexed over the nodes has to be reconstructed from pairwise measurements of differences between its components associated to nodes connected by an edge. In order to model heterogeneity and uncertainty of the measurements, we assume them to be affected by additive noise distributed according to a Gaussian mixture. In this original setup, we formulate the problem of computing the Maximum-Likelihood (ML) estimates and we design two novel algorithms, based on Least Squares regression and Expectation-Maximization (EM). The first algorithm (LS- EM) is centralized and performs the estimation from relative measurements, the soft classification of the measurements, and the estimation of the noise parameters. The second algorithm (Distributed LS-EM) is distributed and performs estimation and soft classification of the measurements, but requires the knowledge of the noise parameters. We provide rigorous proofs of convergence of both algorithms and we present numerical experiments to evaluate and compare their performance with classical solutions. The experiments show the robustness of the proposed methods against different kinds of noise and, for the Distributed LS-EM, against errors in the knowledge of noise parameters.

==> Figures/201610/RandomGraphN15.tex <==
\usetikzlibrary{
arrows, 											%% For Arrows,
decorations.markings ,
positioning,									%% Placing nodes relative to other nodes
% external, 										%% Provides a high-level automatic or semi-automatic export feature for TikZ pictures
}
% \tikzexternalize								% % Activate

% \tikzset
% {
% vertex/.style = 
% 	{
% 	shape = circle, 		% % Node Shape
% 	style = semithick, 	% % Node Style
% 	draw = blue!50, 		% % Node Color
% 	fill = blue!20, 		% % Node Filling
% 	inner sep = 0pt, 		% % Inner Separation between Text and Shape
% 	minimum size = 5mm, 	% % Minimum Height and Width; For circle it is the radius
% 	% % node distance = 1cm, 	% % Node Distance
% 	% %on grid = true
% 	}	% % In order to position Nodes on the grid
% }
% \tikzset
% {
%  big arrow/.style=
%   	{
%     decoration={markings, mark=at position 1 with {\arrow[scale=2,#1]{>}}},
%     postaction={decorate},
%     shorten >=1pt,
%     >= stealth
%     	},
%   big arrow/.default=red!40!white
% }

% Node definition
\tikzstyle{node}=
	[
	shape = circle, 		% % Node Shape
	style = semithick, 	% % Node Style
	draw = blue!50, 		% % Node Color
	fill = blue!20, 		% % Node Filling
	inner sep = 0pt, 		% % Inner Separation between Text and Shape
	minimum size = 5mm, 	% % Minimum Height and Width; For circle it is the radius
	]
	
% Edge definition		
\tikzstyle{edge}=
	[
%     	decoration={markings, mark=at position 1 with {\arrow[scale=2,#1]{>}}},
%     	postaction={decorate},
%     	shorten >=1pt,
%     	>= stealth,
%   	edge/.default=red!40!white
	]

\begin{tikzpicture}[
	xscale	= 2, % to scale horizontally everything but the text
	yscale	= 2, % to scale vertically everything but the text
	]
	% Draw Help Lines
	%%\draw[help lines] (-5, -5) grid (5, 5);
	
	% Number of nodes
	\pgfmathtruncatemacro\nrOfNodes{15}
	
	% Random positioning of nodes
	\foreach \i in {1,...,\nrOfNodes} 
	{
            \pgfmathsetmacro{\posX}{rand*(5)}
            \pgfmathsetmacro\posY{rand*(3)}
            \node[node] (a\i) at (\posX, \posY) {\i};
        }
        
        \def\fromarray
        {
        	{
        	5, 10, 6, 10, 14, 15, 10, 11, 13, 7, 
        	8, 12, 8, 14, 15, 9, 11, 13, 12, 9, 
        	11, 12, 13, 11, 14, 13, 13, 15
        	}
        }
        \def\toarray
        {
        	{
        	1, 1, 2, 2, 2, 2, 3, 3, 3, 4,
        	4, 4, 5, 5, 5, 6, 6, 6, 7, 8,
        	8, 8, 8, 9, 9, 10, 11, 11
        	}
        }
        
        \foreach \y in {0,...,27}
        {
		\pgfmathsetmacro{\j}{array(\fromarray, \y)}
		\pgfmathsetmacro{\i}{array(\toarray, \y)}
        	\draw [edge] 	(a\j) 	to 	(a\i);
        }
        
        
        
	
	
	


	
% 	\node [vertex] (G1) at (-1, 0)		{1};
% 	\node [vertex] (G2) at (0, 0) 		{2};
% 	\node [vertex] (G3) at (1, 1)		{3};
% 	\node [vertex] (G4) at (1, 0)		{4};
% 	\node [vertex] (G5) at (0, -1)		{5};
% 	\draw [big arrow]  	(G2)		to	 node[auto] {$ e_{1} $} (G1);
% 	\draw [big arrow]  	(G3)		to	 node[auto, swap] {$ e_{2} $} (G1);
% 	\draw [big arrow]  	(G4)		to	 node[auto] {$ e_{3} $}	(G2);	
% 	\draw [big arrow]  	(G5)		to	 node[auto] {$ e_{4} $}	(G2);
% 	\draw [big arrow]  	(G4)		to	 node[auto, swap] {$ e_{5} $}	(G3);

\end{tikzpicture}

==> Figures/201610/RandomGraphN50.tex <==
\usetikzlibrary{
arrows, 											%% For Arrows,
decorations.markings ,
positioning,									%% Placing nodes relative to other nodes
% external, 										%% Provides a high-level automatic or semi-automatic export feature for TikZ pictures
}
% \tikzexternalize								% % Activate

% \tikzset
% {
% vertex/.style = 
% 	{
% 	shape = circle, 		% % Node Shape
% 	style = semithick, 	% % Node Style
% 	draw = blue!50, 		% % Node Color
% 	fill = blue!20, 		% % Node Filling
% 	inner sep = 0pt, 		% % Inner Separation between Text and Shape
% 	minimum size = 5mm, 	% % Minimum Height and Width; For circle it is the radius
% 	% % node distance = 1cm, 	% % Node Distance
% 	% %on grid = true
% 	}	% % In order to position Nodes on the grid
% }
% \tikzset
% {
%  big arrow/.style=
%   	{
%     decoration={markings, mark=at position 1 with {\arrow[scale=2,#1]{>}}},
%     postaction={decorate},
%     shorten >=1pt,
%     >= stealth
%     	},
%   big arrow/.default=red!40!white
% }

% Node definition
\tikzstyle{node}=
	[
	shape = circle, 		% % Node Shape
	style = semithick, 	% % Node Style
	draw = blue!50, 		% % Node Color
	fill = blue!20, 		% % Node Filling
	inner sep = 0pt, 		% % Inner Separation between Text and Shape
	minimum size = 5mm, 	% % Minimum Height and Width; For circle it is the radius
	]
	
% Edge definition		
\tikzstyle{edge}=
	[
%     	decoration={markings, mark=at position 1 with {\arrow[scale=2,#1]{>}}},
%     	postaction={decorate},
%     	shorten >=1pt,
%     	>= stealth,
%   	edge/.default=red!40!white
	]

\begin{tikzpicture}[
	xscale	= 2, % to scale horizontally everything but the text
	yscale	= 2, % to scale vertically everything but the text
	]
	% Draw Help Lines
% % 	\draw[help lines] (-5, -5) grid (5, 5);
	
	% Number of nodes
	\pgfmathtruncatemacro\nrOfNodes{50}
	
	% Random positioning of nodes
	\foreach \i in {1,...,\nrOfNodes} 
	{
            \pgfmathsetmacro{\posX}{rand*(5)}
            \pgfmathsetmacro\posY{rand*(5)}
            \node[node] (a\i) at (\posX, \posY) {\i};
        }
        
        \def\fromarray
        {
        	{
18, 24, 32,  8, 13, 45, 50,  5, 15, 21, 22, 39, 43,  6, 10, 12, 13, 16,
29, 41, 43, 47, 26, 31, 45, 49, 27, 47, 25, 31, 34, 48, 10, 39, 40, 43,
41, 19, 20, 25, 36, 46, 20, 22, 36, 48, 32, 46, 26, 45, 49, 18, 28, 43,
45, 34, 46, 21, 41, 46, 23, 27, 36, 39, 41, 42, 44, 33, 34, 47, 33, 36,
50, 28, 45, 37, 44, 35, 44, 47, 42, 35, 32, 36, 40, 42, 46, 41, 46, 49,
43, 45, 46, 37, 40, 45, 40, 41, 48, 40, 49, 42, 43, 44, 46, 47, 50, 47,
50, 50
        	}
        }
        \def\toarray
        {
        	{
1,  1,  1,  2,  2,  2,  2,  3,  3,  3,  3,  3,  3,  4,  4,  4,  4,  4,
4,  4,  5,  5,  6,  6,  6,  6,  7,  7,  8,  8,  8,  8,  9,  9,  9,  9,
10, 11, 11, 11, 11, 11, 12, 12, 12, 12, 13, 13, 14, 14, 14, 15, 15, 15,
15, 16, 16, 17, 17, 17, 18, 18, 18, 18, 18, 18, 18, 20, 20, 20, 21, 23,
23, 24, 24, 25, 25, 26, 26, 26, 27, 29, 30, 30, 30, 31, 31, 33, 34, 34,
35, 35, 35, 36, 36, 36, 37, 37, 37, 38, 39, 40, 40, 40, 43, 43, 44, 46,
46, 49
        	}
        }
        
        \foreach \y in {0,...,109}
        {
		\pgfmathsetmacro{\j}{array(\fromarray, \y)}
		\pgfmathsetmacro{\i}{array(\toarray, \y)}
        	\draw [edge] 	(a\j) 	to 	(a\i);
        }
        
        
        
	
	
	


	
% 	\node [vertex] (G1) at (-1, 0)		{1};
% 	\node [vertex] (G2) at (0, 0) 		{2};
% 	\node [vertex] (G3) at (1, 1)		{3};
% 	\node [vertex] (G4) at (1, 0)		{4};
% 	\node [vertex] (G5) at (0, -1)		{5};
% 	\draw [big arrow]  	(G2)		to	 node[auto] {$ e_{1} $} (G1);
% 	\draw [big arrow]  	(G3)		to	 node[auto, swap] {$ e_{2} $} (G1);
% 	\draw [big arrow]  	(G4)		to	 node[auto] {$ e_{3} $}	(G2);	
% 	\draw [big arrow]  	(G5)		to	 node[auto] {$ e_{4} $}	(G2);
% 	\draw [big arrow]  	(G4)		to	 node[auto, swap] {$ e_{5} $}	(G3);

\end{tikzpicture}

==> Figures/RandomGraphN15.tex <==
\usetikzlibrary{
arrows, 											%% For Arrows,
decorations.markings ,
positioning,									%% Placing nodes relative to other nodes
% external, 										%% Provides a high-level automatic or semi-automatic export feature for TikZ pictures
}
% \tikzexternalize								% % Activate

% \tikzset
% {
% vertex/.style = 
% 	{
% 	shape = circle, 		% % Node Shape
% 	style = semithick, 	% % Node Style
% 	draw = blue!50, 		% % Node Color
% 	fill = blue!20, 		% % Node Filling
% 	inner sep = 0pt, 		% % Inner Separation between Text and Shape
% 	minimum size = 5mm, 	% % Minimum Height and Width; For circle it is the radius
% 	% % node distance = 1cm, 	% % Node Distance
% 	% %on grid = true
% 	}	% % In order to position Nodes on the grid
% }
% \tikzset
% {
%  big arrow/.style=
%   	{
%     decoration={markings, mark=at position 1 with {\arrow[scale=2,#1]{>}}},
%     postaction={decorate},
%     shorten >=1pt,
%     >= stealth
%     	},
%   big arrow/.default=red!40!white
% }

% Node definition
\tikzstyle{node}=
	[
	shape = circle, 		% % Node Shape
	style = semithick, 	% % Node Style
	draw = blue!50, 		% % Node Color
	fill = blue!20, 		% % Node Filling
	inner sep = 0pt, 		% % Inner Separation between Text and Shape
	minimum size = 5mm, 	% % Minimum Height and Width; For circle it is the radius
	]
	
% Edge definition		
\tikzstyle{edge}=
	[
%     	decoration={markings, mark=at position 1 with {\arrow[scale=2,#1]{>}}},
%     	postaction={decorate},
%     	shorten >=1pt,
%     	>= stealth,
%   	edge/.default=red!40!white
	]

\begin{tikzpicture}[
	xscale	= 2, % to scale horizontally everything but the text
	yscale	= 2, % to scale vertically everything but the text
	]
	% Draw Help Lines
	%%\draw[help lines] (-5, -5) grid (5, 5);
	
	% Number of nodes
	\pgfmathtruncatemacro\nrOfNodes{15}
	
	% Random positioning of nodes
	\foreach \i in {1,...,\nrOfNodes} 
	{
            \pgfmathsetmacro{\posX}{rand*(5)}
            \pgfmathsetmacro\posY{rand*(3)}
            \node[node] (a\i) at (\posX, \posY) {\i};
        }
        
        \def\fromarray
        {
        	{
        	5, 10, 6, 10, 14, 15, 10, 11, 13, 7, 
        	8, 12, 8, 14, 15, 9, 11, 13, 12, 9, 
        	11, 12, 13, 11, 14, 13, 13, 15
        	}
        }
        \def\toarray
        {
        	{
        	1, 1, 2, 2, 2, 2, 3, 3, 3, 4,
        	4, 4, 5, 5, 5, 6, 6, 6, 7, 8,
        	8, 8, 8, 9, 9, 10, 11, 11
        	}
        }
        
        \foreach \y in {0,...,27}
        {
		\pgfmathsetmacro{\j}{array(\fromarray, \y)}
		\pgfmathsetmacro{\i}{array(\toarray, \y)}
        	\draw [edge] 	(a\j) 	to 	(a\i);
        }
        
        
        
	
	
	


	
% 	\node [vertex] (G1) at (-1, 0)		{1};
% 	\node [vertex] (G2) at (0, 0) 		{2};
% 	\node [vertex] (G3) at (1, 1)		{3};
% 	\node [vertex] (G4) at (1, 0)		{4};
% 	\node [vertex] (G5) at (0, -1)		{5};
% 	\draw [big arrow]  	(G2)		to	 node[auto] {$ e_{1} $} (G1);
% 	\draw [big arrow]  	(G3)		to	 node[auto, swap] {$ e_{2} $} (G1);
% 	\draw [big arrow]  	(G4)		to	 node[auto] {$ e_{3} $}	(G2);	
% 	\draw [big arrow]  	(G5)		to	 node[auto] {$ e_{4} $}	(G2);
% 	\draw [big arrow]  	(G4)		to	 node[auto, swap] {$ e_{5} $}	(G3);

\end{tikzpicture}
